An Extensible Benchmark Suite for Learning to Simulate Physical Systems

Simulating physical systems is a core component of scientific computing, encompassing a wide range of physical domains and applications. Recently, there has been a surge in data-driven methods to complement traditional numerical simulations methods, motivated by the opportunity to reduce computational costs and/or learn new physical models leveraging access to large collections of data. However, the diversity of problem settings and applications has led to a plethora of approaches, each one evaluated on a different setup and with different evaluation metrics. We introduce a set of benchmark problems to take a step towards unified benchmarks and evaluation protocols. We propose four representative physical systems, as well as a collection of both widely used classical time integrators and representative data-driven methods (kernel-based, MLP, CNN, nearest neighbors). Our framework allows evaluating objectively and systematically the stability, accuracy, and computational efficiency of data-driven methods. Additionally, it is configurable to permit adjustments for accommodating other learning tasks and for establishing a foundation for future developments in machine learning for scientific computing.

==> macros.tex <==
% Some macro definitions here

\usepackage{amssymb, amsthm, amsfonts, amsmath}
\usepackage{mathtools, mathrsfs}
\usepackage{xparse}
% So we can use @ in internal commands
\makeatletter

\newcommand{\@bbset}[2]{\newcommand{#1}{\ensuremath{\mathbb{#2}}}}
\@bbset{\bbR}{R}
\@bbset{\bbQ}{Q}
\@bbset{\bbC}{C}
\@bbset{\bbZ}{Z}
\@bbset{\bbN}{N}
\@bbset{\bbF}{F}

\newcommand{\hsep}{\centerline{\noindent\rule[0.5ex]{0.5\textwidth}{0.5pt}}}

% Define delimiter pairs
\DeclarePairedDelimiter\dparen{\lparen}{\rparen}
\DeclarePairedDelimiter\dbrace{\lbrace}{\rbrace}
\DeclarePairedDelimiter\dbrack{\lbrack}{\rbrack}
\DeclarePairedDelimiter\dangle{\langle}{\rangle}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Probability-related macros
\DeclareMathOperator{\Exp}{E}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\pr}{\Pr}

% Probability distributions
\DeclareMathOperator{\pbern}{Bern} % Bernoulli
\DeclareMathOperator{\pbinom}{Binom} % Binomial
\DeclareMathOperator{\pbeta}{Beta} % Beta
\DeclareMathOperator{\pdir}{Dir} % Dirichlet
\DeclareMathOperator{\pnorm}{\mathcal{N}} % Normal/Gaussian
\DeclareMathOperator{\pgam}{Gam} % Gamma
\DeclareMathOperator{\pstut}{St} % Student-t
\DeclareMathOperator{\deltat}{\delta t}

% Vector and matrix operators
\NewDocumentCommand\evec{m}{\mathbf{#1}}
\NewDocumentCommand\emat{m}{\mathbf{#1}}

% Put @ back where it was before
\makeatother

\newcommand{\DP}[1]{\textcolor{red}{DP: #1}}
\newcommand{\JB}[1]{\textcolor{cyan}{JB: #1}}
\newcommand{\BP}[1]{\textcolor{magenta}{BP: #1}}
\newcommand{\AG}[1]{\textcolor{orange}{AG: #1}}
\newcommand{\DZ}[1]{\textcolor{purple}{DZ: #1}}
\newcommand{\KO}[1]{\textcolor{blue}{KO: #1}}
\newcommand{\TS}[1]{\textcolor{green}{TS: #1}}

